The Inadequacy of Shapley Values for Explainability

This paper develops a rigorous argument for why the use of Shapley values in explainable AI (XAI) will necessarily yield provably misleading information about the relative importance of features for predictions. Concretely, this paper demonstrates that there exist classifiers, and associated predictions, for which the relative importance of features determined by the Shapley values will incorrectly assign more importance to features that are provably irrelevant for the prediction, and less importance to features that are provably relevant for the prediction. The paper also argues that, given recent complexity results, the existence of efficient algorithms for the computation of rigorous feature attribution values in the case of some restricted classes of classifiers should be deemed unlikely at best.

==> tabs/tab-bf-stats.tex <==
\begin{table}[t]
  %\begin{center}
  \centering{
    \renewcommand{\arraystretch}{1.15}
    \renewcommand{\tabcolsep}{0.5em}
    \begin{tabular}{lr}
      \toprule
      Total number of functions & 65536 \\
      Total number of instances & 1048576 \\
      \midrule
      Total number of I1a issues & 781696 \\
      Number of functions with I1a issues & 65320 \\
      \% I1a issues / function & 99.67 \\
      \midrule
      Total number of I1b issues & 105184 \\
      Number of functions with I1b issues & 40448 \\
      \% I1b issues / function & 61.72 \\
      Max number of swaps & 3 \\
      Avg number of swaps & 1.36 \\
      \midrule
      Total number of I2 issues & 43008 \\
      Number of functions with I2 issues & 7800 \\
      \% I2 issues / function & 11.90 \\
      \midrule
      Total number of I3 issues & 5728 \\
      Number of functions with I3 issues & 2592 \\
      \% I3 issues / function & 3.96 \\
      \bottomrule
    \end{tabular}
    %
    %\begin{tabular}{lr}
    %\toprule
    %Total number of functions &  65536 \\
    %Total number of instances & 1048576 \\
    %\midrule
    %Total number of I1 issues & 781696 \\
    %Number of function-distinct I1 issues & 65320 \\
    %\% I1 issues / function & 99.67 \\
    %\midrule
    %Total number of I2 issues & 43008 \\
    %Number of function-distinct I2 issues & 7800 \\
    %\% I2 issues / function & 11.90 \\
    %\midrule
    %Total number of I3 issues & 5728 \\
    %Number of function-distinct I3 issues & 2592 \\
    %\% I3 issues / function &  3.96 \\
    %\bottomrule
    %\end{tabular}
  }
  %\end{center}
  \caption{Some statistics for functions with 4 variables}
  \label{tab:bf-stats}
\end{table}


==> tabs/tab-sumup.tex <==
\begin{table}[t]
  %\begin{center}
  \centering{
    \renewcommand{\tabcolsep}{0.375em}
    \begin{tabular}{ccccccc} \toprule
      Dataset & Features &
      \%{\spc}Out{\spc}of{\spc}Order &
      \%{\spc}$\exists${\spc}R{\spc}in{\spc}Bot$K$ & \%{\spc}Maj{\spc}R{\spc}in{\spc}Bot$K$ & 
      \%{\spc}$\exists${\spc}I{\spc}in{\spc}Top$K$ & \%{\spc}Maj{\spc}I{\spc}in{\spc}Top$K$ \\
      \toprule 
      corral & 6 &
      26.2 & 0.0 & 0.0 & 26.2 & 26.2 \\
      %
      mux6 & 6 &
      56.8 & 30.8 & 30.8 & 0.0 & 0.0 \\
      %
      threeOf9 & 9 &
      56.8 & 24.2 & 4.4 & 28.0 & 0.0 \\
      %
      xd6 & 9 &
      54.2 & 51.8 & 20.4 & 45.4 & 25.4 \\
      %
      mofn\_3\_7\_10 & 10 &
      44.4 & 0.0 & 0.0 & 33.4 & 0.0 \\
      %
      parity5+5 & 10 &
      34.2 & 11.6 & 0.2 & 0.0 & 0.0 \\
      \bottomrule
    \end{tabular}
  }
  %\end{center}
  \caption{Summary of results.
    \%{\spc}Out{\spc}of{\spc}Order denotes the percentage of instances with out of
    order irrelevant features, i.e.\ there exist some irrelevant
    feature(s) with a Shapley value (or score) greater than the
    Shapley value of some relevant feature(s);
    %
    \%{\spc}$\exists${\spc}R{\spc}in{\spc}Bot$K$ denotes the percentage of instances with
    relevant features having some of the $K$ smallest scores (and 
    which have at least one irrelevant feature that has a larger
    score);
    %
    \%{\spc}Maj{\spc}R{\spc}in{\spc}Bot$K$ denotes the percentage of instances with relevant
    features representing the majority of the $K$ smallest scores (and
    which have at least one irrelevant feature that has a larger
    score);
    %
    \%{\spc}$\exists${\spc}I{\spc}in{\spc}Top$K$ denotes the percentage of instances with
    irrelevant features having some of the $K$ largest scores (and 
    which have at least one relevant feature that has a smaller
    score);
    %
    \%{\spc}Maj{\spc}I{\spc}in{\spc}Top$K$ denotes the percentage of instances with
    irrelevant features representing the majority of the $K$ largest
    scores (and which have at least one relevant feature that
    has a smaller score);
    %
    $K$ is 2 for datasets with 6 features, and 3 for the other
    datasets.}
  \label{tab:sumup}
\end{table}

